Structured Stochastic Gradient MCMC

Stochastic gradient Markov Chain Monte Carlo (SGMCMC) is considered the gold standard for Bayesian inference in large-scale models, such as Bayesian neural networks. Since practitioners face speed versus accuracy tradeoffs in these models, variational inference (VI) is often the preferable option. Unfortunately, VI makes strong assumptions on both the factorization and functional form of the posterior. In this work, we propose a new non-parametric variational approximation that makes no assumptions about the approximate posterior's functional form and allows practitioners to specify the exact dependencies the algorithm should respect or break. The approach relies on a new Langevin-type algorithm that operates on a modified energy function, where parts of the latent variables are averaged over samples from earlier iterations of the Markov chain. This way, statistical dependencies can be broken in a controlled way, allowing the chain to mix faster. This scheme can be further modified in a "dropout" manner, leading to even more scalability. We test our scheme for ResNet-20 on CIFAR-10, SVHN, and FMNIST. In all cases, we find improvements in convergence speed and/or final accuracy compared to SG-MCMC and VI.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/old_algo2.tex <==

  
  \KwIn{Initial sample $\theta^{(0)}$; parameter partitions $\theta_1,\dots,\theta_M$; step sizes $\{\epsilon_t\}_{t=0,\dots,T-1}$.}
  \KwOut{$\hat{q}^{(T)}(\theta) := \{\theta^{(t)}\}_{t=1,\dots,T}$}
  \For{$t = 0$ to $T-1$}{
    Sample minibatch $\tilde{\mathcal{D}}^{(t)} \subset \mathcal{D}$\;
    \For{$i=1$ to $M$}{
        Sample $\tilde{\theta}_{\lnot i}^{(t)} \sim \hat{q}_{\lnot i}^{(t)}$\;
        $\hat{U}_i^{(S, t)} = \hat{U}([\theta^{(t)}_i, \tilde{\theta}^{(t)}_{\lnot i}]; \tilde{\mathcal{D}}^{(t)})$\!\!\!\!
    }
    $\nabla_\theta \hat{U}^{(S, t)} = \sum_{i=1}^M \nabla_\theta \hat{U}_i^{(S, t)}$\!\!\!\!\!\!\!\!\;
    $\theta^{(t+1)} =$ \texttt{SGMCMC\_step}$(\theta^{(t)}, \nabla_\theta \hat{U}^{(S, t)},\epsilon_t)$
  }
 

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \KwIn{Initial sample $\theta^{(0)}$; parameter partitions $\theta_1,\dots,\theta_M$; data set $\mathcal{D}$; initial auxiliary statistics $\xi^{(0)}$; step sizes $\{\epsilon_t\}_{t=1,\dots,T}$; masking distribution $p^{(S_d)}$; dropout iterations $K$.}
  \KwOut{$\hat{q}^{(T)}(\theta) := \{\theta^{(t)}\}_{t=1,\dots,T}$}
  \For{$t = 0$ to $T-1$}{
    Sample minibatch $\tilde{\mathcal{D}}^{(t)} \subset \mathcal{D}$\;
    \For{$k=1$ to $K$}{ 
        Sample masks $r^{(t,k)}_{1}, \dots, r^{(t,k)}_{M} \sim p^{(S_d)}$\;
        Sample $\tilde{\theta}^{(t,k)} \sim \hat{q}^{(t)}$\;
        $\theta^{(t,k)} = [r^{(t,k)}_{i}\theta^{(t)}_i + (1-r^{(t,k)}_{i})\tilde{\theta}_i^{(t,k)}]_{i=1,\dots,M}$\;
        $\hat{U}_k^{(S_d, t)} = \hat{U}(\theta^{(t,k)}; \tilde{\mathcal{D}}^{(t)})$ \;
    }
    ${\nabla}_\theta \hat{U}^{(S_d, t)} = \frac{M}{K\mathbb{E}_{r\sim p^{(S_d)}}\left[\sum_{i=1}^M r_i\right]} \sum_{k=1}^K \nabla_\theta \hat{U}_k^{(S_d, t)}$ \;
    $\theta^{(t+1)}, \xi^{(t+1)} = \texttt{SGMCMC\_step}(\theta^{(t)}, {\nabla}_\theta \hat{U}^{(S_d, t)}, \xi^{(t)},\epsilon_t)$
  }
 


==> sections/old_method.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\normalem

% Introduce data and Introduce posterior energy function for Bayesian deep learning
Given data $\mathcal{D}=\{(x_i,y_i)\}_{i=1,\dots,N}$, parameters $\theta$, a proper prior distribution $p(\theta)$, and a likelihood $p(\mathcal{D}|\theta) = \prod_{i=1}^N p(y_i|x_i,\theta)$, suppose we are interested in the corresponding posterior distribution $p(\theta|\mathcal{D})\propto p(\mathcal{D}|\theta)p(\theta)$. A convenient representation of the posterior is as a Boltzmann distribution:
\begin{align}
p(\theta|\mathcal{D})  \propto \exp\{-U(\theta)\} 
\;\;\text{ where }\;\; U(\theta)  = -\sum_{(x,y)\in \mathcal{D}} \log p(y|x,\theta) - \log p(\theta). \label{eq:energy_dist}
\end{align}
$U$ is typically referred to as the \emph{posterior energy function}. Note that the posterior distribution is typically intractable due to the normalizing constant. 

% Define MAP
Should the \emph{maximum a posteriori} (MAP) of $\theta$ (i.e., $\argmax_\theta p(\theta|\mathcal{D})$) be desired, it can be found directly with $\hat\theta_{\text{MAP}} = \argmin_\theta U(\theta)$ via various optimization methods, such as SGD. While the MAP is typically quick to optimize for, it does not afford uncertainty estimates of $\theta$ or any downstream usages of $\theta$ (e.g., such as predictive uncertainty). 

The gold standard for approximating the entire posterior distribution is by deploying Markov chain Monte Carlo (MCMC) algorithms. These methods work by producing an empirical distribution of samples through a random walk in parameter space. While being very accurate and having asymptotic guarantees, these methods are known to not scale well with respect to both data and parameters \citep{brooks2011handbook,geyer1992practical}.

% Define different sg-mcmc algorithms
Stochastic gradient MCMC (SGMCMC) is a class of scalable MCMC algorithms that is able to produce posterior samples through the use of gradients on minibatches of data.
%rather than gradients on the entire set of data.
These algorithms are largely derived from discretized approximations of continuous-time diffusion processes. Examples of these algorithms include stochastic gradient Langevin dynamics (SGLD) \citep{welling2011bayesian}, preconditioned SGLD (pSGLD) \citep{li2016preconditioned}, and stochastic gradient Hamiltonian Monte Carlo (SGHMC) \citep{chen2014stochastic}.

As alluded to, the basis of SGMCMC algorithms is using a sampled minibatch of data $\tilde{\mathcal{D}}$ from $\mathcal{D}$ to produce an unbiased estimate of the gradient of the posterior energy function:
\begin{align}
    \nabla_\theta U(\theta) &\approx \hat \nabla_\theta U(\theta) =: N\nabla_\theta G(\theta;\tilde{\mathcal{D}})\\
\text{where }    G(\theta;\tilde{\mathcal{D}}) &= -\frac{1}{|\tilde{\mathcal{D}}|} \sum_{(x,y)\in\tilde{\mathcal{D}}} \log p(y|x,\theta) - \frac{1}{N} \log p(\theta). \label{eq:energy_approx}
\end{align}
$G(\cdot)$ can be seen as representing a normalized minibatch loss (with regularization from the prior). Different algorithms use this gradient approximation in different ways to propose new samples of $\theta$ in their random walks. The update rules for SGLD, pSGLD, and SGHMC are defined as follows:
\begin{align}
\text{SGLD} \;\; \theta^{(t+1)} & = \theta^{(t)} -\frac{\epsilon_t}{2}\hat \nabla_\theta U(\theta^{(t)}) + \mathcal{N}(0,\epsilon_t I) \label{eq:sgld}\\
\text{pSGLD} \;\; \theta^{(t+1)} & = \theta^{(t)} -\frac{\epsilon_t}{2}\left[R(\theta^{(t)})\hat \nabla_\theta U(\theta^{(t)}) + \sum_\theta \nabla_\theta R(\theta^{(t)})\right] + \mathcal{N}(0, \epsilon_t R(\theta^{(t)})) \label{eq:psgld}\\
\text{SGHMC} \;\; \theta^{(t+1)} & =\theta^{(t)} + \epsilon_t M^{-1}m^{(t+1)} \\
m^{(t+1)} & = (1-\gamma\epsilon_t M^{-1})m^{(t)} - \epsilon_t \hat \nabla_\theta U(\theta^{(t)}) + \mathcal{N}(0, 2\gamma-\epsilon_t\hat V(\theta^{(t)})) \label{eq:sghmc}
\end{align}
where $\epsilon_t$ is the step size at time step $t$, $R(\cdot)$ and $M$ are preconditioners, $\gamma \geq 0$ is a friction term, and $\hat V(\cdot)$ is an estimate of the covariance induced by the stochastic gradient.\footnote{Note that we abuse notation in Eqs.~\ref{eq:sgld}-\ref{eq:sghmc} where the addition of $\mathcal{N}(\mu,\Sigma)$ denotes the addition of a normally distributed random variable with mean $\mu$ and covariance $\Sigma$.} All of these methods produce a \emph{chain} of samples up to time step $t$ that ultimately form an empirical distribution $\hat p^{(t)}(\theta | \mathcal{D})$. Should the algorithms converge, then $\lim_{t\rightarrow \infty} \hat p^{(t)}(\theta | \mathcal{D}) = p(\theta | \mathcal{D})$.


\section{Structured SGMCMC}
\label{sec:method}

% Derive variational sg-mcmc setup (in general)
By design, SGMCMC methods produce a completely joint posterior distribution over parameters $\theta$. For models with a large amount of parameters, this can lead to various complications due to the curse of dimensionality. This is typically seen with slow convergence times and potentially unexplored parameter spaces. A viable solution is to break dependencies in the posterior distribution by leveraging variational inference (VI). This would reduce the number of various potential posterior correlations that the model would need to capture while sampling.

To do so, we first start by partitioning the parameters into $M>1$ distinct groups: $\theta_1, \dots, \theta_M$. The structured, approximate posterior distribution will be denoted as $q(\theta) = \prod_{i=1}^M q_i(\theta_i)$; however, it should be noted that unlike traditional VI, we are \textbf{not} assuming a parametric form of $q$ --- only structural. $q(\theta)$ is encouraged to best approximate the posterior $p(\theta|\mathcal{D})$ by seeking to minimize the KL-divergence between the two:
\begin{align}
J(q(\theta)) % & = J(q_1(\theta_1), \dots, q_M(\theta_M)) \\ 
&= D_\text{KL}(q(\theta) || p(\theta|\mathcal{D}))  \\
& \equiv \mathbb{E}_{\theta\sim q}\left[\log \frac{q(\theta)}{p(\theta|\mathcal{D})}\right] \label{eq:kl}
\end{align}

\cref{thm:kl_min} proves that there is a unique solution to the KL minimization problem described in \cref{eq:kl}, and it defines $U^{(S)}$ which allows us to use SGMCMC to approximate the posterior $q(\theta)$ with samples. This Theorem will later present ALGORITHM that actually approximate this distribution $q(\theta)$, resulting in a new non-parametric VI scheme.

\begin{theorem}
The unique solution to the KL minimization problem given in Eq.~\ref{eq:kl} is given by the Boltzmann distribution $Z^{-1}  \exp\{-\sum_{i=1}^M U_i^{(S)}(\theta_i)\}$ where $U_i^{(S)}(\theta_i)=\mathbb{E}_{\tilde{\theta}_{\lnot i} \sim q_{\lnot i}}[\log p(\theta_i, \tilde{\theta}_{\lnot i}, \mathcal{D})]$ for $i=1,\dots,M$ and $Z$ is a normalizing constant. 
\label{thm:kl_min}
\end{theorem}
\vspace{-1em}
% \begin{proof}
% We begin by rewriting Eq.~\ref{eq:kl} as follows: 
% \begin{flalign}
%     J&(q(\theta)) = \E_{\theta \sim q}\left[\log q(\theta)\right] - \E_{\theta \sim q}\left[\log \prob(\theta, \mathcal{D})\right] + C\\
% %    & = \E_{\theta \sim q}\left[\log \prob(\theta, \mathcal{D})\right] - \E_{\theta_i \sim q_i}\left[\log q_i(\theta_i)\right] - \sum_{i\neq j}\E_{\theta_j \sim q_j}\left[\log q_j(\theta_j)\right] \\
% %& = \int \log p(\theta, \mathcal{D}) q(\theta) d\theta - \E_{\theta_i \sim q_i}\left[\log q_i(\theta_i)\right] - \sum_{i\neq j}\E_{\theta_j \sim q_j}\left[\log q_j(\theta_j)\right] \\
%     =& \E_{\theta_i \sim q_i}\left[\log q_i(\theta_i)\right] + \sum_{i\neq j}\E_{\theta_j \sim q_j}\left[\log q_j(\theta_j)\right] - \int \log p(\theta, \mathcal{D}) q_i(\theta_i)d\theta_i \prod_{i\neq j} q_j(\theta_j)d\theta_j + C
% \end{flalign}
% for some $i \in \{1, \dots, M\}$ where $\lnot i := \{1, \dots, M\} \setminus \{i\}$ and $C=\log p(\mathcal{D})$. In order to find the optimal distribution that respects the factorization constraints imposed between parameter groups, we need to minimize this functional over $q$ --- or rather every $q_i$. This is done by taking the functional derivative of $J$ with respect to $q_i$, setting it equal to zero, and solving for $q_i$:
% \begin{align}
%     \frac{\delta J(q(\theta))}{\delta q_i(\theta_i)} & = \int \log p(\theta, \mathcal{D}) \prod_{i\neq j} q_j(\theta_j)d\theta_j  - 1 - \log q_i(\theta_i) := 0 \\ 
%     \implies \log q_i(\theta_i) & = \E_{\tilde{\theta}_{\lnot i} \sim q_{\lnot i}}\left[\log p(\theta_i, \tilde{\theta}_{\lnot i}, \mathcal{D})\right] - 1 \\
% %    \implies q_i(\theta_i) & = e^{\E_{\theta_{\lnot i} \sim q_{\lnot i}}\left[\log p(\theta_i, \theta_{\lnot i}, \mathcal{D})\right] - 1} \\
%     \implies q_i(\theta_i) & \propto \exp\left\{\E_{\tilde{\theta}_{\lnot i} \sim q_{\lnot i}}\left[\log p(\theta_i, \tilde{\theta}_{\lnot i}, \mathcal{D})\right]\right\}. \label{eq:vi_dist}
% \end{align}
% By defining the energy $U^{(\text{V})}_i(\theta_i) = -\E_{\tilde{\theta}_{\lnot i} \sim q_{\lnot i}}\left[\log p(\theta_i, \tilde{\theta}_{\lnot i}, \mathcal{D})\right]$, we realize that by minimizing the KL-divergence in Eq.~\ref{eq:kl}, the approximate posterior distribution $q=\prod_{i=1}^M q_i$ takes the form of a Boltzmann distribution as in Eq.~\ref{eq:energy_dist} with $U^{(\text{V})}(\theta)=\sum_{i=1}^M U^{(\text{V})}_i(\theta_i)$.

% It remains to be shown that the solution is unique. To this end, we refer to the convexity of the KL divergence in function space \citep{doi:https://doi.org/10.1002/0471200611.ch2}. This implies that the stationary point of the KL is indeed a global optimum and unique. \qedhere
% \end{proof}
We will now show how to leverage the results of \cref{thm:kl_min} to construct an algorithm that can produce samples from the approximate posterior $q(\theta)$. Since $U^{(S)}$ is properly defined, samples that approximate $q(\theta)$ can be generated using SGMCMC algorithms. Similar to $\hat{p}^{(t)}(\theta|\mathcal{D})$, we will denote the empirical distribution of samples up to time step $t$ from $q(\theta)$ as $\hat{q}^{(t)}(\theta)$. The only requirement is to use these algorithms to define the stochastic estimate of the energy function's gradient $\hat{\nabla}_\theta U^{(S)}(\theta)$:
\begin{align}
\nabla_\theta U^{(S)}(\theta) & \approx \hat{\nabla}_\theta U^{(S)}(\theta) =: N \nabla_\theta G^{(S)}(\theta; \tilde{\mathcal{D}}) \\
 G^{(S)}(\theta; \tilde{\mathcal{D}}) & = \sum_{i=1}^M \mathbb{E}_{\tilde{\theta}_{\lnot i} \sim q_{\lnot i}} G(\{\theta_i, \tilde{\theta}_{\lnot i}\}; \tilde{\mathcal{D}}) \label{eq:var_sum}
%\text{where } G_i^{(S)}(\theta_i; \tilde{\mathcal{D}}) & = -\mathbb{E}_{\theta_{\lnot i} \sim q_{\lnot i}} \left[\frac{1}{|\tilde{\mathcal{D}}|}\sum_{(x,y)\in\tilde{\mathcal{D}}} \log p(y|x,\theta_i,\theta_{\lnot i}) + \frac{1}{N} \log p(\theta_i,\theta_{\lnot i})\right].
\end{align}
%where $[\cdot]$ indicates combining the given parameter group arguments and ``unpartitions'' them into the original form of $\theta$. 
In practice, $\mathbb{E}_{\tilde{\theta}_{\lnot i} \sim q_{\lnot i}} G(\{\theta_i, \tilde{\theta}_{\lnot i}\}; \tilde{\mathcal{D}})$ is approximated using a single-sample, Monte Carlo estimate:
\begin{align}
\mathbb{E}_{\tilde{\theta}_{\lnot i} \sim q_{\lnot i}} G(\{\theta_i^{(t)}, \tilde{\theta}_{\lnot i}\}; \tilde{\mathcal{D}}) & \approx G(\{\theta^{(t)}_i, \tilde{\theta}^{(t)}_{\lnot i}\}; \tilde{\mathcal{D}}) \label{eq:v_g}
%- \frac{1}{|\tilde{\mathcal{D}}|}\sum_{(x,y)\in\tilde{\mathcal{D}}} \log p(y|x,\theta^{(t)}_i,\tilde{\theta}^{(t)}_{\lnot i}) + \frac{1}{N} \log p(\theta^{(t)}_i,\tilde{\theta}^{(t)}_{\lnot i}), \\
%\text{where } \tilde{\theta}^{(t)}_{\lnot i} &:= \{\tilde{\theta}^{(t)}_j\}_{j\neq i} \text{ with } \tilde{\theta}^{(t)}_j \sim \hat{q}_j^{(t)}(\theta_j), \label{eq:v_sub}
\end{align}
where $\tilde{\theta}^{(t)}_i$ is sampled from the chain $\hat{q}^{(t)}_i$. 
Putting \cref{eq:v_g} into words, the minibatch loss specific to $\theta_i^{(t)}$ is approximated by substituting $\theta_{\lnot i}^{(t)}$ in the model with a sample from the empirical approximate posterior $\hat{q}_{\lnot i}^{(t)}$. 

While a formal proof of convergence needs to be shown, one can see that the approximate posterior is a fixed point of the sampling scheme. Namely, if $q_{\lnot i}(\theta_{\lnot i})$ is stationary, then the Monte-Carlo gradient of \cref{eq:v_g} with respect to $\theta_i$ will be an unbiased gradient estimator of the energy function's true gradient \cref{eq:var_sum} and the Langevin chain will converge to the correct marginal, and in particular \emph{remain} stationary. In practice, we find that the scheme converges to a stationary distribution (\cref{sec:experiments}).


This formulation of $\hat \nabla_\theta U^{(S)}(\theta)$ can be plugged in anywhere $\hat \nabla_\theta U(\theta)$ appears in the original SGMCMC algorithms. The resulting class algorithms will be referred to as structured SGMCMC (S-SGMCMC). We will denote specific structured variants of SGMCMC algorithms with a `S' prefix (e.g., S-SGLD, S-pSGLD, and S-SGHMC). The full algorithm can be seen in Algorithm~\ref{alg:vsgmcmc}.

\section{Structured Dropout SGMCMC}
\label{sec:method_dropout}
% Discuss how it is further possible to generalize S-SGMCMC by deriving an encompassing class of energy functions.
With just a slight shift in perspective, it is actually possible to further generalize $U^{(S)}$ (and consequently S-SGMCMC) to produce a broader class of approximate sampling algorithms.
This is done by first noting that $U^{(S)}$ can be represented with a scaled double-expectation:
\begin{align}
U^{(S)}(\theta) = -\frac{M}{\E_{r\sim p^{(S)}}\left[\sum_{i=1}^M r_i\right]} E_{r\sim p^{(S)}}E_{\tilde{\theta} \sim q} \left[\log p(r\theta + (1-r)\tilde{\theta}, \mathcal{D})\right] \label{eq:u_exp}
\end{align}
where $p^{(S)}(r) = \text{Cat}(r; M^{-1},\dots,M^{-1})$ and $(r\theta + (1-r)\tilde{\theta})_i$ is equal to $\theta_i$ if $r_i = 1$ and $\tilde{\theta}_i$ otherwise for $i=1,\dots,M$. Note that this is constructed in this manner specifically so that $U^{(S)}$ remains differentiable with respect to $\theta$. Also note that though the denominator appears superfluous as $\E_{r\sim p^{(S)}}[\sum_{i=1}^M r_i] = 1$, it is necessary for certain theoretic properties, as seen in \cref{thm:limit_case}.

By replacing $p^{(S)}$ with a more flexible distribution, we can further generalize and encapsulate different energy functions to sample from. One such choice is $p^{(S_d)}(r;\rho) :\propto \prod_{i=1}^M\text{Bern}(r_i;\rho)\ind(\sum_{i=1}^M r_i > 0)$ with $\rho \in (0,1)$.\footnote{Other choices of distribution that are well justified include any with support over $[0,1]^M$ and with measure 0 over $\{0\}^M$. Exploring the effects these distributions have are an interesting line of future inquiry.} 
Substituting $p^{(S)}$ for $p^{(S_d)}$ in \cref{eq:u_exp} yields a new energy function that we will refer to as $U^{(S_d)}$.
We note that this choice in distribution leads to a dropout-like behavior \citep{nalisnick2019dropout,srivastava2014dropout}, where the composition of model parameters as $r\theta+(1-r)\tilde{\theta}$ leads to each parameter group $\theta_i$ having a probability of approximately $\rho$ to be used in a prediction and a $(1-\rho)$ probability of being replaced by $\tilde{\theta}_i$ from the approximate posterior (in traditional dropout, $\theta_i$ would instead be replaced with 0).
Likewise, we will denote methods that use this energy function for sampling as structured dropout SGMCMC (S$_d$-SGMCMC) with different variants all sharing the same S$_d$ prefix (e.g. S$_d$-SGHMC).

\begin{theorem} \label{thm:limit_case}
For a given set of parameters $\theta$ partitioned into $M$ groups, the following holds true: (i) $U^{(S_d)} \rightarrow U$ as $\rho \rightarrow 1$ and (ii) $U^{(S_d)} \rightarrow U^{(S)}$ as $\rho \rightarrow 0$. Thus, distributions approximated by S$_d$-SGMCMC lie on a continuum with those generated by S-SGMCMC at one extreme and with those from SGMCMC at the other.
\end{theorem}
\vspace{-0.7em}
Please refer to the Supplement for the full, formal proof. Informally, a dropout rate of $\rho=1$ implies that $r\theta + (1-r)\tilde{\theta}$ is equivalent to just $\theta$. This, in effect, recovers the original energy function $U$ as every parameter group is updated together. Likewise, when $\rho \rightarrow 0$ it can be shown that $p^{(S_d)}(r_i=1,r_{\lnot i}=0; \rho) \rightarrow M^{-1}$ for $i=1,\dots,M$. As such, this implies that $p^{(S_d)} \rightarrow \text{Cat}(M^{-1},\dots,M^{-1})$ which in turn recovers $U^{(S)}$ from $U^{(S_d)}$ by design.

In practice, the double-expectation in $U^{(S_d)}$ is jointly approximated using a Monte Carlo estimate with $K$ samples. This leads to the following approximated gradients to use with SGMCMC algorithms:
\begin{align}
\nabla_\theta U^{(S_d)}(\theta^{(t)}) & \approx \hat{\nabla}_\theta U^{(S_d)}(\theta^{(t)}) =: N \nabla_\theta G^{(S_d)}(\theta^{(t)}; \tilde{\mathcal{D}}) \\
G^{(S_d)}(\theta^{(t)}; \tilde{\mathcal{D}}) & \approx \frac{1}{K\rho}\sum_{k=1}^K G(r^{(t,k)}\theta^{(t,k)} + (1-r^{(t,k)})\tilde{\theta}^{(t,k)}; \tilde{\mathcal{D}}) \label{eq:dropout_scale}
\end{align}
where $r^{(t,k)} \sim p^{(S_d)}$ and $\tilde{\theta}^{(t,k)} \sim \hat{q}^{(t)}$ for $k=1,\dots,K$.
We note that by approximating $U^{(S_d)}$ in this way, computing a gradient no longer scales on the order of $\mathcal{O}(M)$, but rather $\mathcal{O}(K)$. This means that the choice of structure imposed on the posterior distribution remains independent of computing resources. As such, configurations with large amounts of parameter groups are typically only feasible when using S$_d$-SGMCMC as S-SGMCMC would use too much memory and/or compute per sample. 



%One drawback to S-SGMCMC is that the computational cost of producing a single sample grows on the order of $\mathcal{O}(M)$ due to the summation in Eq.~\ref{eq:var_sum}. Instead of calculating the minibatch loss specific to one particular parameter group, the same gradients can be approximated by calculating the minibatch loss with respect to a random subset of parameter groups. Taking inspiration from dropout, let $\rho \in (0,1)$ be the probability of a parameter group being selected for a single iteration. With this setup, iterations are not tied to specific parameter groups so this effectively decouples the number of minibatch losses computed from the number of parameter groups. Let $K\geq 1$ be the number of iterations computed per sample. This method will be denoted by `S$_d$', either stand alone or as a prefix to SGMCMC algorithms (e.g., S$_d$-SGLD, S$_d$-pSGLD, and S$_d$-SGHMC).

% More formally, we can compose the effective weights that a model will use for iterations $k=1,\dots,K$ like so:
% \begin{align}
% \theta^{(t,k)} & = [\theta^{(t,k)}_i]_{i=1,\dots,M} \label{eq:dropout_comp1}\\ \theta_{i}^{(t,k)} & = r_{k,i} \theta_{i}^{(t)} + (1-r_{k,i})\widetilde \theta^{(t,k)}_i \label{eq:dropout_comp2}
% \end{align}
% where  $r_{k,i} \sim \text{Bernoulli}(\rho)$ and $\widetilde \theta^{(t,k)}_i \sim \hat{q}_i^{(t)}(\theta_i)$.\footnote{For optimal theoretic properties, the sampled values of $r_{k,i}$ must also have a restriction that $\sum_{i=1}^M r_{k,i} \neq 0$ thus making $r_{k,i}$ not exactly independent and identically distributed Bernoulli random variables. In practice, this restriction is not used due to typically having a large value of $\mathbb{E}[\sum_{i=1}^M r_{k,i}]=M\rho$.} With these compositions, the gradients of variational posterior energy function during sampling are approximated like so:
% \begin{align}
% \hat{\nabla}_\theta U^{(S)}(\theta^{(t)}) & \approx \hat{\nabla}_\theta U^{(S_d)}(\theta^{(t)}) := N \nabla_\theta G^{(S_d)}(\theta^{(t)}; \tilde{\mathcal{D}}) \\
% G^{(S_d)}(\theta^{(t)}; \tilde{\mathcal{D}}) & \approx \frac{1}{K\rho}\sum_{k=1}^K G(\theta^{(t,k)}; \tilde{\mathcal{D}}). \label{eq:dropout_scale}
% \end{align}
% Due to the sampling procedure in Eqs.~\ref{eq:dropout_comp1}-\ref{eq:dropout_comp2}, the gradient for $\theta_i$ will not be masked out on average $K\rho$ of $K$ total iterations. As such, we scale by $\frac{1}{K\rho}$ in Eq.~\ref{eq:dropout_scale} to adjust for this. Note that for brevity we have only shown the resulting Monte Carlo estimate of $G^{(S_d)}$, and in turn of $U^{(S_d)}$. Please refer to the Supplement for the full specification and derivation, as well as the algorithm for S$_d$-SGMCMC.

% \begin{theorem} \label{thm:limit_case}
% For a given set of parameters $\theta$ partitioned into $M$ groups, the following holds true: (i) $U^{(S_d)} \rightarrow U$ as $\rho \rightarrow 1$ and (ii) $U^{(S_d)} \rightarrow U^{(S)}$ as $\rho \rightarrow 0$. Thus, distributions approximated by S$_d$-SGMCMC lie on a continuum with those generated by S-SGMCMC at one extreme and with those from SGMCMC at the other.
% \end{theorem}
% \vspace{-0.7em}
% Please refer to the Supplement for the proof of \cref{thm:limit_case}. 

\begin{table}
\begin{tabular}{@{}c@{}c@{}}
\raisebox{0.08cm}{\begin{minipage}{.43\textwidth}
\input{sections/algo1}
\end{minipage}}& \hspace{0.005\textwidth} 
\begin{minipage}{.555\textwidth}
\centering
\input{sections/experiment_table}
\end{minipage}
\end{tabular}
\end{table}
% \end{minipage}
% \begin{minipage}[t]{0.4\textwidth}
%   \vspace{0pt}
% \input{sections/experiment_table}
% \end{minipage}


% Consider parameters $\theta$ (which is a vector containing $P$ parameters) with prior distribution $p(\theta)$ and dataset $\mathcal{D}$ containing data $X_1, \dots, X_N$. For simplicity, we will assume prior independence amongst all $\theta$. Assume independence between data points and that each has a differentiable likelihood $p(X_i | \theta)$. We \sout{wish}\tonycomment{want}\todo{I don't think that wish sounds that good here} to find the posterior distribution $p(\theta | \mathcal{D})$. 

% This can be achieved by using a stochastic gradient Markov chain Monte-Carlo (SG-MCMC) algorithm. An example of one is stochastic gGradient Langevin dynamics (SGLD) which composes a Markov chain of posterior samples using the following update rule:
% \begin{align*}
% \theta^{(t+1)} = \theta^{(t)} + \frac{\epsilon_t}{2}\left(\nabla_\theta \log p(\theta^{(t)}) + \frac{N}{n} \sum_{i=1}^n \nabla_\theta \log p(X_{t_i} | \theta^{(t)}) \right) + \eta_t
% \end{align*}
% where $\eta_t \sim \mathcal{N}(0, \epsilon_t)$.

% We can impose independence assumptions between specific parameters. Assume that we group parameters into $M$ groups $\theta_1, \dots, \theta_M$ such that $\cup_{i=1}^M \theta_i = \theta$ and $\theta_i \cap \theta_j = \emptyset$ for $i \neq j$ (i.e. they partition the original parameter space with $M \leq P$). Thus, we would like to approximate the true posterior distribution $\prob(\theta | \mathcal{D})$ with $q(\theta) = \prod_{i=1}^M q_i(\theta_i)$. This is accomplished by optimizing the evidence lower bound (ELBO), like so:

% \begin{align*}
%     J( & q(\theta))  = J(q_1(\theta_1), \dots, q_M(\theta_M)) \\
%     & = \E_{\theta \sim q}\left[\log \frac{\prob(\theta, \mathcal{D})}{q(\theta)}\right] \\
%     & = \E_{\theta \sim q}\left[\log \prob(\theta, \mathcal{D})\right] - \E_{\theta \sim q}\left[\log q(\theta)\right] \\
% %    & = \E_{\theta \sim q}\left[\log \prob(\theta, \mathcal{D})\right] - \E_{\theta_i \sim q_i}\left[\log q_i(\theta_i)\right] - \sum_{i\neq j}\E_{\theta_j \sim q_j}\left[\log q_j(\theta_j)\right] \\
% %& = \int \log p(\theta, \mathcal{D}) q(\theta) d\theta - \E_{\theta_i \sim q_i}\left[\log q_i(\theta_i)\right] - \sum_{i\neq j}\E_{\theta_j \sim q_j}\left[\log q_j(\theta_j)\right] \\
%     & = \int \log p(\theta, \mathcal{D}) q_i(\theta_i)d\theta_i \prod_{i\neq j} q_j(\theta_j)d\theta_j  - \E_{\theta_i \sim q_i}\left[\log q_i(\theta_i)\right] - \sum_{i\neq j}\E_{\theta_j \sim q_j}\left[\log q_j(\theta_j)\right] \\
% \end{align*}
% for some $i \in \{1, \dots, M\}$. Taking the functional derivative and setting equal to zero yields the following:

% \begin{align*}
%     \frac{\delta J(q(\theta))}{\delta q_i(\theta_i)} & = \int \log p(\theta, \mathcal{D}) \prod_{i\neq j} q_j(\theta_j)d\theta_j  - 1 - \log q_i(\theta_i) := 0 \\
%     \implies \log q_i(\theta_i) & = \E_{\theta_{\lnot i} \sim q_{\lnot i}}\left[\log p(\theta_i, \theta_{\lnot i}, \mathcal{D})\right] - 1 \\
%     \implies q_i(\theta_i) & = e^{\E_{\theta_{\lnot i} \sim q_{\lnot i}}\left[\log p(\theta_i, \theta_{\lnot i}, \mathcal{D})\right] - 1} \\
%     \implies q_i(\theta_i) & \propto e^{\E_{\theta_{\lnot i} \sim q_{\lnot i}}\left[\log p(\theta_i, \theta_{\lnot i}, \mathcal{D})\right]} \\
% \end{align*}


% Using the imposed independence structures on the parameters groups, we can find approximate posterior distributions via the following update equations that are put into effect simultaneously:

% \begin{align*}
%     \theta^{(t+1)}_j & = \theta^{(t)}_j + \frac{\epsilon_t}{2}\left(\nabla_{\theta_j} \log p(\theta^{(t)}) + \frac{N}{n} \sum_{i=1}^n \nabla_{\theta_j} \log p(X_{t_i} | \theta^{(t)}_j, \widetilde \theta^{(t)}_{\lnot j}) \right) + \eta_t, \\
% \end{align*}
% for $j\in \{1, \dots, M\}$ where $\widetilde \theta^{(t)}_{\lnot j} \equiv \{\widetilde \theta^{(t)}_{1}, \dots, \widetilde \theta^{(t)}_{j-1}, \widetilde \theta^{(t)}_{j+1}, \dots, \widetilde \theta^{(t)}_{M}\}$ with $\widetilde \theta^{(t)}_{j}$ being a sample of the $j^\text{th}$ parameter group taken from the approximate posterior chain at time step $t$ (i.e., $\widetilde \theta^{(t)}_{j} \sim \widetilde q^{(t)}(\theta_j)$) Note that $\widetilde \theta^{(t)}_{j}$ is not the same as the current state $\theta^{(t)}_j$.

% Computing these equations primarily involves computing the following loss function
% $$
% \sum_{j=1}^M \sum_{i=1}^n \log p(X_{t_i} | \theta^{(t)}_j, \widetilde \theta^{(t)}_{\lnot j})
% $$
% which requires computing $M$ forward passes through the model \sout{(}\tonycomment{,}assuming we can parallelize over the batch dimension $i$\sout{)}.

% \section{Dropout Variational SG-MCMC}

% Taking inspiration from the section above, we can similarly structure the model's parameters into $M$ separate groups; however, we will not strictly enforce the structured independence between them. Instead, for a given iteration, we will have $K$ forward passes where in each pass every parameter group will have a $\gamma \in (0, 1)$ probability of using the most current value instead of being sampled.

% More formally, let 

% \begin{align*}
% \theta_{j}^{(t,k)} & = \rho_{k,j} \theta_{j}^{(t)} + (1-\rho_{k,j})\widetilde \theta^{(t,k)}_j \\
% \text{where } & \rho_{k,j} \sim \text{Bernoulli}(\gamma) \text{ and } \widetilde \theta^{(t,k)}_j \sim \widetilde q^{(t)}(\theta_j)
% \end{align*}
% for $k \in \{1,\dots,K\}$ and $j\in \{1,\dots,M\}$. $\gamma$ will be referred to as the dropout rate\footnote{Note that $\gamma = 1$ yields the same update rule as regular SG-MCMC algorithms}. Following the same inspiration from the structured SG-MCMC, the update rule is as follows:

% \begin{align*}
% \theta^{(t+1)} = \theta^{(t)} + \frac{\epsilon_t}{2}\left(\nabla_\theta \log p(\theta^{(t)}) + \frac{N}{nK\gamma} \sum_{k=1}^K \sum_{i=1}^n \nabla_\theta \log p(X_{t_i} | \theta^{(t,k)}) \right) + \eta_t
% \end{align*}
% where $\theta^{(t,k)}$ is a vector composed of $\theta^{(t,k)}_j$ for $j\in\{1,\dots,M\}$. The double sum is scaled by $\frac{N}{nK\gamma}=\frac{N}{n}\frac{1}{K\gamma}$. The first term is to account for the difference in size between the sampled batch and the dataset. The second term is average the gradient over the $K$ multiple forward passes, but also scale up the signal by $\gamma^{-1} > 1$ to account for a parameter group not always having a gradient for each forward pass (i.e., for $K$ forward passes, a parameter group is expected to have a gradient calculated for them in $K\gamma$ of them).

==> sections/related-work-OLD.tex <==
\section{Related Work}
\label{sec:related}

%Despite MCMC's practicality and simplicity it is a demanding algorithm in both computational power and time. A new family of algorithms was introduced in order to make MCMC more scalable, the Stochastic Gradient Markov Chain Monte-Carlo (SG-MCMC).

Our work connects both to (stochastic) variational inference 
\citep{bishop2006pattern,hoffman2013stochastic,ranganath2014black,blei2017variational,zhang2018advances} and scalable MCMC \citep{welling2011bayesian,chen2014stochastic,ma2017stochastic,zhang2019cyclical,leimkuhler2019partitioned}. While much of this work would have deserved discussions, for space limitations, we focus our discussion on the most related work at the intersection of both lines of works. 

%While there has been much work on scalable MCMC (\cite{welling2011bayesian}, \cite{robbins1951stochastic},\cite{li2016preconditioned}, \cite{hoffman2020black}, \cite{chen2014stochastic}, \cite{ma2017stochastic}, \cite{heek2019bayesian}, \cite{leimkuhler2019partitioned}, \cite{zhang2019cyclical}, \cite{mandt2017stochastic}, \cite{NIPS2013_309928d4}) and variational inference (\cite{bishop2006pattern}, \cite{hoffman2013stochastic}, \cite{hoffman2015structured}, \cite{wang2013variational}, \cite{tierney1989fully}, \cite{mackay1992information}, \cite{bickel2007mathematical}, \cite{ranganath2014black}, \cite{ranganath2013adaptive}, \cite{nalisnick2019dropout}), we will focus on works that draw connections on both methods.



% \paragraph{Scalable MCMC} Proposed by \cite{welling2011bayesian}, stochastic gradient Langevin dynamics (SGLD) is one of the simplest and easiest to implement example of SG-MCMC methods. Inspired by stochastic gradient descent (SGD) \citep{robbins1951stochastic}, it introduces the addition of Gaussian noise in the SGD updates enabling SGLD to find the exact posterior distribution. Preconditioned SGLD, a modification of SGLD, was introduced by \cite{li2016preconditioned} who combined preconditioners with SGLD in order to tackle the rapidly changing curvature in parameter space which renders default SGLD methods inefficient. \cite{hoffman2020black} suggested that the transient bias of Langevin dynamics may track that of variational inference (VI) due to the fact that Markov chains have not burned it and that the optimizer in VI has not converged yet. Their theoretical analysis proves that you can get more accurate results by running a MCMC procedure than a VI procedure. \cite{chen2014stochastic} proposed \sout{a new stochastic gradient approach based on Hamiltonian dynamical systems,} the stochastic gradient Hamiltonian Monte-Carlo (SG-HMC) algorithm\sout{. SG-HMC}\tonycomment{, which} introduces a variant that uses second-order Langevin dynamics with a friction term that counteracts the effects of the noisy gradient, maintaining the desired target distribution as the invariant distribution. \cite{ma2017stochastic} \sout{came up with SG-MCMC Methods for Hidden Markov Models. They consider a marginal likelihood representation of the HMM and their method harnesses the inherent memory decay of the process.} \tonycomment{considering a marginal likelihood representation of the HMM they came up with SG-MCMC Methods for Hidden Markov Models which harnesses the inherent memory decay of the process.} \cite{leimkuhler2019partitioned} employed thermodynamic parameterization methods that improve neural network training while the partitioning of parameters enables rapid convergence\sout{. Their work involved}\tonycomment{, involving} easy-to-implement hybrid partitioned numerical algorithms that are based on discretized stochastic differential equations. \cite{heek2019bayesian} introduced \sout{an }adaptive noise MCMC (ATMC) algorithm \sout{that estimates and is able to sample from the posterior of a Bayesian neural network. ATMC} \tonycomment{which }adjusts the amount of momentum and noise applied to the parameter updates in order to compensate for the stochastic gradients \tonycomment{and is able to sample from the posterior of a Bayesian neural network}. \cite{zhang2019cyclical} developed Cyclical Stochastic SG-MCMC with a cyclical stepsize schedule\sout{, where larger steps discover new modes, and smaller steps characterize each mode. They demonstrate the scalability and effectiveness of their proposed method in learning complex multimodal distributions} by replacing the traditional decreasing stepsize schedule in SG-MCMC with a cyclical variant. \cite{mandt2017stochastic} proposed \sout{a scalable approximate MCMC algorithm,} the averaged stochastic gradient sampler and provided various contributions on scalable MCMC algorithms. \cite{NIPS2013_309928d4} \sout{showed the importance of} Riemannian geometry \sout{of the simplex} in \sout{designing} Langevin MCMC algorithms\sout{. In this new method which they call}\tonyadjusts{with} stochastic gradient Riemannian Langevin dynamics\sout{ they use a mirroring trick to remove boundaries, coupled with a natural gradient update.}\tonycomment{ which coupled with a natural gradient update removes boundaries.}


% \paragraph{Variational Inference} On the other hand we have variational inference (VI) an \sout{another} approximate posterior inference algorithm with supplementary strengths to MCMC. While MCMC is computationally expensive and asymptotically exact, VI is fast and comes without warranties. A large variety of VI methods has emerged throughout the years. \cite{bishop2006pattern} proposed coordinate ascent mean-field variational inference which iteratively optimizes each parameter while holding the others fixed in a mean-field fashion. \cite{hoffman2013stochastic} developed Stochastic Variational Inference(SVI)\sout{, a stochastic optimization algorithm for mean-field variational inference,} which is a scalable modification to Variational Bayes harnessing stochastic gradients. The limitations of SVI were surpassed by Structured Stochastic Variational Inference(SSVI) proposed by \cite{hoffman2015structured}. SSVI is a generalization of SVI that restores the dependence between local and global parameters while at the same time it avoids the local optima \sout{and the sensitivity of hyperparameter tuning that limits the Mean Field Variational Inference(MFVI).} \cite{wang2013variational} presented two generic methods to MFVI for nonconjugate models, Laplace Variational Inference and delta method variational inference. The former uses Laplace approximations(\cite{tierney1989fully}, \cite{mackay1992information}) in a variational optimization algorithm. The latter optimizes a Taylor approximation of the variational objective\sout{, which produces an alternative interpretation of Laplace variational inference or it uses a multivariate delta approximation (\cite{bickel2007mathematical}) of the variational objective}. Moreover \cite{ranganath2014black} introduced Black Box Variational Inference(BBVI), where the noisy gradient of a stochastic optimization of the variational objective is computed from Monte Carlo samples from the variational distribution. BBVI reduces the variance of the gradient, while at the same time it avoids difficult model-based derivations. \cite{ranganath2013adaptive} developed an adaptive learning rate for stochastic variational inference, which is easy to implement and does not require \sout{any} tuning. \cite{nalisnick2019dropout} proposed a novel method for understanding multiplicative noise in neural networks considering dropout, and showing that dropout’s Monte Carlo training objective approximates marginal MAP estimation.

% \paragraph{Hybrid Methods} 
There are algorithms that serve both as hybrids combining MCMC and VI into one method with interpolation schemes. \cite{domke2017divergence} proposes a divergence bound for hybridizing VI and MCMC, essentially by running Langevin dynamics on a tempered ELBO. \cite{de2001variational} proposed a mixture of a random walk Metropolis kernel and a block Metropolis-Hastings(MH) kernel with a variational approximation as proposal distribution. An improved approach to that was introduced by \cite{habib2018auxiliary} where by introducing low dimensional auxiliary variables they fit a more accurate approximating distribution\sout{ and leverage the learned low dimensional structure to take very large steps in the target space}. \cite{salimans2015markov} \sout{describe theoretical foundations in order to combine IV and MCMC. They }argued that integrating one or more MCMC steps into the approximation can improve variational inference. \cite{liu2014projecting} \sout{gave sufficient conditions to guarantee that univariate Gibbs sampling on Markov Random Fields (MRFs) will be fast mixing. They }suggested projecting the parameters of an MRF onto the set of fast-mixing parameters, for which MCMC quickly converges to the true distribution. \cite{ahn2012bayesian} came up with Stochastic Gradient Fisher Scoring which interpolates between Langevin dynamics and a Gaussian approximation of the target and involves a Gaussian approximation of the posterior target to derive approximate MCMC updates. \cite{domke2014projecting} projected Ising model parameters onto a parameter set that is guaranteed to be fast mixing, under several divergences. \sout{They also found that Gibbs sampling using the projected parameters is more accurate when interaction strengths are strong and when limited time is available for sampling.} \cite{rezende2015variational} interpreted the path of an MCMC algorithm as a variational distribution, and then fitting parameters to tighten a variational bound. To the best of our knowledge our proposal is the first one to introduce a dropout inspired hybrid SGMCMC algorithm which interpolates between MCMC and VI.

% \paragraph{Scalable MCMC}
% \begin{itemize}
%     \item SG-Langevin Dynamics
%     \item SG-HMC
%     \item Fancy schemes as introduced in cold posterior paper [Leimkuhler]
%     \item A complete recipe of SG-MCMC [Emily Fox]...
% \end{itemize}
% \paragraph{Variational Inference}
% \begin{itemize}
%     \item Coordinate-ascent variational inference (Bishop 2006)
%     \item Non-parametric Variational Inference..?
%     \item...
% \end{itemize}
% \paragraph{Hybrid Methods}
% \begin{itemize}
%     \item Justin Domke?
%     \item...
% \end{itemize}
